Enhancing Large-Scale AI Training Efficiency: The C4 Solution for Real-Time Anomaly Detection and Communication Optimization

The emergence of Large Language Models (LLMs) has necessitated the adoption of distributed training techniques, involving the deployment of thousands of GPUs to train a single model. Unfortunately, the efficiency of large-scale distributed training systems is often suboptimal due to the increased likelihood of hardware errors in high-end GPU products and the heightened risk of network traffic collisions. Moreover, any local hardware failure can disrupt training tasks, and the inability to swiftly identify faulty components leads to a significant waste of GPU resources. And, prolonged communication due to traffic collisions can substantially increase GPU waiting times. To address these challenges, we propose a communication-driven solution, namely the C4. The key insights of C4 are twofold. First, the load in distributed training exhibits homogeneous characteristics and is divided into iterations through periodic synchronization, therefore hardware anomalies would incur certain syndrome in collective communication. By leveraging this feature, C4 can rapidly identify the faulty components, swiftly isolate the anomaly, and restart the task, thereby avoiding resource wastage caused by delays in anomaly detection. Second, the predictable communication model of collective communication, involving a limited number of long-lived flows, allows C4 to efficiently execute traffic planning, substantially reducing bandwidth competition among these flows. The C4 has been extensively deployed across real-world production systems in a hyperscale cloud provider, yielding a significant improvement in system efficiency, from 30% to 45%. This enhancement is attributed to a 30% reduction in error-induced overhead and a 15% reduction in communication costs.

==> tex/design_path.tex <==

\subsection{Network load-balancing in collective communication}
Synchrony is a key aspect of collective communication in LLM training. During a collective communication, each GPU sends and receives messages. The communication finishes only after all messages are successfully delivered. Therefore, traffic of a collective communication should be evenly distributed across network, to prevent congestion in a part of network paths, which slows down the whole communication process.

However, in GPU cluster networks, inter-host routing often relies on hashing (e.g., ECMP protocol), which itself can create uneven network traffic distribution, leading to congestion on a part of links. Further, link failures or background traffic may also exacerbate this congestion.

To mitigate the congestion caused by load imbalance, we make three design choices. (1) We developed rProbe for real-time network monitoring. (2) Based on the monitoring result of rProbe, we modified NCCL's queue pair (QP) establish process to utilize all available network path, and avoid all network links in trouble. (3) We modified NCCL's data chunk allocation method among QPs to ensure load balancing during communication. Figure~\ref{?} illustrates our design.

\textbf{rProbe.}
In the ECMP (Equal-Cost Multi-Path) protocol, given the IP addresses of the sender and receiver, based on the source port number, the hash-based algorithm allows the ToR (Top-of-Rack) switch to select different Spine Switches for forwarding, thereby enabling different forwarding paths. rProbe constructs probe messages and enumerates source ports. Utilizing the INT (In-band Network Telemetry) protocol, it identifies all available paths and broken paths in the current network from the current IP to any other IP, as well as the specific source port numbers that will enable the ECMP protocol to accurately route to these paths.

\textbf{Network-aware QP establishment.}
Based on rProbe, we identify the number of Spine Switches in the current network and the correspondence between source port numbers and these switches. Consequently, in NCCL's QP establishment, we modify the source port for each QP to ensure an even distribution across all Spine Switches in the network. For example, suppose an NCCL communication channel has $N$ QPs and rProbe detects $M$ Spine Switches in the network, then the $i$th QP will be mapped to the Spine Switch of ID $i$ \% $M$.
Similarly, if the network provides multiple ToR (Top-of-Rack) switches for a single network interface card (NIC), we set the transmit affinity (TXA) to evenly distribute these QPs across all available ToR switches. 
This design tries to distribute different QPs to different network paths, to fully utilize the cluster network.

\textbf{Balancing QP workload during communication.}
During NCCL communication, data chunks are distributed to multiple QPs for transmission. Due to network heterogeneity or competition from other traffic in the network, the bandwidth of each QP may be different, resulting in different queue lengths. We modify NCCL's data chunk allocation strategy, so that given a data chunk, the QP with the shortest current queue length is selected. This ensures that all QPs can complete the data transmission approximately at the same time.
